Billiards Sports Analytics: Datasets and Tasks

Nowadays, it becomes a common practice to capture some data of sports games with devices such as GPS sensors and cameras and then use the data to perform various analyses on sports games, including tactics discovery, similar game retrieval, performance study, etc. While this practice has been conducted to many sports such as basketball and soccer, it remains largely unexplored on the billiards sports, which is mainly due to the lack of publicly available datasets. Motivated by this, we collect a dataset of billiards sports, which includes the layouts (i.e., locations) of billiards balls after performing break shots, called break shot layouts, the traces of the balls as a result of strikes (in the form of trajectories), and detailed statistics and performance indicators. We then study and develop techniques for three tasks on the collected dataset, including (1) prediction and (2) generation on the layouts data, and (3) similar billiards layout retrieval on the layouts data, which can serve different users such as coaches, players and fans. We conduct extensive experiments on the collected dataset and the results show that our methods perform effectively and efficiently.

==> eval_similarity.tex <==
\subsection{Evaluation on the Billiards Layout Retrieval Task}
\label{subsec:similar}

\subsubsection{Experimental Setup}
\label{sec:setup}

\if 0
\begin{table}[t]
\centering
%\setlength{\abovecaptionskip}{1pt}
\caption {Dataset statistics.} \label{tab:dataset}
\setlength{\tabcolsep}{5.3mm}{
\begin{tabular}{c|c}
\hline
% \textbf{Dataset}               & \textbf{Statistics}                                 \\
\hline
\#layouts                         & 3019                                               \\
\#games                       & 94                                             \\
\#players                      & 227                                           \\
year                        & 2020 - 2020                                           \\
\#clear labels (or not)     & 1,217 (1,802)                                           \\
\#win labels (or not)       & 1,295 (1,724)                                           \\
x-axis & {[}0,200{]}\\
y-axis & {[}0,100{]}\\
\hline
\end{tabular}}
\vspace{-2mm}
\label{tab:stat}
\end{table}

\noindent \textbf{Dataset.}
We collected a real-world billiards layouts dataset, which consists of 3,019 break shots in 94 international professional 9-ball games played by 227 players in recent 20 years (i.e., 2020-2020). 
\if 0
We give more details on the dataset as follows.%~\cite{pan2021development}

When we collect data, a perspective grid provided by the software Kinovea is used on the closed surface of the table which is calibrated into a $200 \times 100$ coordinate system. The coordinates generally belong to the $[0, 200]$ range along the x-axis, and the $[0, 100]$ range along the y-axis, with the left bottom corner of the table being $(0,0)$.
\fi
% The information we collect includes 
For each layout, we have the positions of balls that remain on the pool table after the break shot, the number of potted balls after the break shot, a binary tag indicating clear or not (clear if the player who performs the break shot pocketed all balls and thus win the game; unclear otherwise), win or not (in a 9-ball game, win if the player potted ball 9 into the pocket, not win otherwise), and remarks. Remarks are used to capture some special situations, such as golden break, which means the ball 9 is potted into a pocket in the break shot; a foul shot, which means the shot is not making the first contact with the lowest numbered ball in the layout, and it is regarded as breaking the rule of competition. In addition, we provide the YouTube video link for each layout.
In the dataset, there are 1,216 (resp. 1,295) billiards layouts with the label ``clear'' (resp. ``win'').
% , which can be found on YouTube. 
%record the source of the layout such as "2019 Men's Diamond Las Vegas Open" and provide video link,  We shall publish the dataset and the codes once the paper is accepted.
{\ChengComment{We note that collecting the data from real sports players but not simulation tools has the following advantages. (1) In most cases, the data is used for applications concerning real games, for which, it is more desirable to use data from real games than from simulation tools. For example, for the score prediction task in practice, it would be more effective to train a model based on data from real games~\cite{aoki2017luck}. (2) For applications concerning real players such as player performance study and play tactics discovery, a common practice is to use data from real players but not that from simulation tools~\cite{decroos2018automatic,pan2021development}.}} 
The dataset statistics is presented in Table~\ref{tab:stat}.
\fi

\begin{figure*}[ht]
\centering
\begin{tabular}{c c}
  \begin{minipage}{8.5cm}%5.5
    \includegraphics[width=16.5cm]{figures/legend}
  \end{minipage}
  &
  \\
   \begin{minipage}{0.42\linewidth}%5.5
    \includegraphics[width=\linewidth]{figures/hr_noise}
    \end{minipage}
    &
    \begin{minipage}{0.42\linewidth}
    \includegraphics[width=\linewidth]{figures/mr_noise}
    \end{minipage}
    \\
    (a) Varying noise rate (HR@10)%\hspace{-4mm}
    &
    (b) Varying noise rate (MRR)%\hspace{-4mm}
    \\
    \begin{minipage}{0.42\linewidth}
    \includegraphics[width=\linewidth]{figures/hr_drop}
    \end{minipage}
    &
    \begin{minipage}{0.42\linewidth}
    \includegraphics[width=\linewidth]{figures/mr_drop}
    \end{minipage}
    \\
    (c) Varying drop rate (HR@10)%\hspace{-4mm}
    &
    (d) Varying drop rate (MRR)%\hspace{-4mm}
\end{tabular}
\vspace{-3mm}
%\setlength{\abovecaptionskip}{1pt}
{\extension{\caption{Effectiveness evaluation (similarity search).}}}
\label{fig:effectiveness_similarity}
\vspace*{-3mm}
\end{figure*}

\noindent \textbf{Baseline.}
To evaluate the effectiveness and efficiency of our BL2Vec, we compare it with the following baselines: %(1) EMD~\cite{rubner2000earth}, (2) Hausdorff~\cite{huttenlocher1993comparing}, (3) DTW~\cite{yi1998efficient}, (4) Frechet~\cite{alt1995computing}, (5) Peer Matching (PM), (6)DeepSets~\cite{zaheer2017deep}, (7) RepSet~\cite{skianis2020rep} and (8) WSSET~\cite{Arsomngern2021self} as discussed in Section~\ref{sec:related}.
%\begin{itemize}
\\
$\bullet$
%\item 
EMD~\cite{rubner2000earth}. The Earth Mover's Distance (EMD) is based on the idea of a transportation problem that measures the least amount of work needed to transform one set to another. %a well-known measurement for pointsets  Besides, EMD is widely used for various applications such as document classification, image retrieval, etc.
\\
$\bullet$
Hausdorff~\cite{huttenlocher1993comparing}. Hausdorff distance is based on the idea of point-matching and computes the largest distance among all the distances from a point in one set to the nearest point in the other set.
\\
$\bullet$
DTW~\cite{yi1998efficient} and Frechet~\cite{alt1995computing}. DTW and Frechet are two widely used similarity measurements for 
sequence data.
%trajectory/time series analysis. Specifically, Frechet is
%a metric, namely the distance is symmetric and satisfies the triangle inequality; however, DTW is not a metric, since it does not satisfy the triangle inequality.
%
To apply the measurements to billiards layouts, we model each layout as a sequence of locations, which corresponds to one cue ball followed by several object balls in ascending order of ball numbers.
\\
$\bullet$
Peer Matching (PM). We adopt a straightforward solution for measuring the similarity between two billiards layouts as the average of the distances between their balls matched based on the numbers, e.g., ball 1 in one layout is matched to the ball 1 in another layout, and so on.
For those mismatched balls with different numbers, we align them in the ascending order of their numbers and match them accordingly.
%}
\\
$\bullet$
DeepSets~\cite{zaheer2017deep}. DeepSets is used to generate pointsets representation in an unsupervised fashion. The main idea of DeepSets is to transform vectors
of points in a set into a new representation of the set. It aggregates the representations of vectors and then passes them to fully-connected layers to get the representation.
\\
$\bullet$
RepSet~\cite{skianis2020rep}. RepSet is also used to generate the representations of pointsets. It adapts a bipartite matching idea by computing the correspondences between an input set and some generated hidden sets to get the set representation. Besides, RepSet captures the unordered nature of a set and can generate the same output for all possible permutations of points in the set.
\\
$\bullet$
WSSET~\cite{Arsomngern2021self}. WSSET achieves the state-of-the-art performance on pointsets embedding, which is an approximate version of EMD based on the deep metric learning framework and uses the EMD as a metric for inferring the positive and negative pairs. It generates the representations of pointsets, and these generated representations can be used for similarity search, classification tasks, etc.
%\end{itemize}

\noindent \textbf{Parameter Setting.}
% We set the cell size to be 15. 
Intuitively, with the smaller cell size, it generates more tokens and provides a higher resolution of the pool table. However, with the smaller size, it reduces the robustness against the noise for the similarity search task. The parameter is set to 15 because it provides better performance in general via empirical studies (with the results of its effect shown later on), and thus %The results and detailed description are included in the technical report~\cite{TR} due to the page limit), % (with the results of its effect shown later on) 
we have 99 unique tokens for the BS features. For BP and BB features, {\ICDEComment{we vary the parameter of angle (resp. distance) from $5^\circ$ to $20^\circ$ (resp. 5 to 20), and since the results are similar, we use the setting of $15^\circ$ and 10 for partitioning the angle range and distance range, respectively.}}
%
For each feature, we embed it to a 10-dimensional vector, and thus the representation dimension of the ball is $10*(1+4*6+2)=270$ (i.e., $K'=270$). Recall that for each ball, there is one token in the BS feature, four tokens in the BP feature with totally six pockets, and two tokens in the BB feature.We use a convolutional layer as $Net(\cdot)$ with 3 output channels. For each, it has 52 filters with varying sizes from $(1,K')$ to $(7,K')$. Note that larger filters help capture the correlations between the balls. A ReLU function is applied after the convolutional layer and then a global max-pooling layer is employed to generate a 156-dimensional representation of the billiards layout (i.e., $K=3 \times 52 = 156$). Additionally, in the training process, we randomly sample 70\% billiards layouts to generate training tuples and adopt Adam stochastic gradient descent with an initial learning rate of $0.00001$, and the remaining layouts are used for testing. To avoid overfitting, we employ a L2 regularization term with $\lambda=0.001$ for $Net(\cdot)$. The margin in the triplet loss is set to $\delta = 1.0$ based on empirical findings.For generating each $\mathcal{B}_+$ (resp. $\mathcal{B}_-$), we set both the noise rate and the drop rate to 0.2 by default. For parameters of baselines, we follow their settings in the original papers.

\noindent \textbf{Evaluation Metrics.}
We consider the following three tasks to evaluate the effectiveness.
(1) Similarity search, we report the Hitting Ratio for Top-10 ($HR@10$) and Mean Reciprocal Rank ($MRR$). In particular, for a query billiards layout $\mathcal{B}_q$, if its positive version $\mathcal{B}_+$ is in the top-10 returned billiards layouts, then $HR@10$ is defined as $HR@10 = 1$, otherwise $HR@10 = 0$.
%
$MRR$ is defined as $MRR = \frac{1}{rank}$, where $rank$ denotes the rank of $\mathcal{B}_+$ in the database for its query billiards layout $\mathcal{B}_q$. The average results of $HR@10$ and $MRR$ over all queries are reported in the experiments. A higher $HR@10$ or $MRR$ indicates a better result.
%
(2) Classification, we report the average classification accuracy for the label of ``clear'' and ``not clear''. 
% "clear" or "not clear".
Classification accuracy is a widely used metric in the classification task. A higher accuracy indicates a better result.
%
(3) Clustering, we report two widely used metrics Adjusted Rand Index (ARI) and Adjusted Mutual Information (AMI) for clustering. %{\color{blue} ~\cite{rand1971objective} ~\cite{vinh2010information}
They measure the correlation between the predicted result and the ground truth. The ARI and AMI values lie in the range $[-1, 1]$. For ease of understanding, we normalize the values in the range of $[0,1]$.
%as a percentage value. %{\color{blue}
A higher ARI or AMI indicates a higher correspondence to the ground-truth.%}

\noindent \textbf{Evaluation Platform.}
All the methods are implemented in Python 3.8. The implementation of $BL2Vec$ is based on PyTorch 1.8.0. The experiments are conducted on a server with 10-cores of Intel(R) Core(TM) i9-9820X CPU @ 3.30GHz 64.0GB RAM and one Nvidia GeForce RTX 2080 GPU. The datasets and codes can be downloaded via the link~\footnote{\url{https://www.dropbox.com/sh/644aceaolfv4rky/AAAKhpY1yzrbq9-uo4Df3N0Oa?dl=0}}.

\if 0
\begin{figure*}[h]
% \vspace*{-2mm}
% \hspace{-2mm}
%\hspace*{-.3cm}
\centering
\begin{tabular}{c c c c}
  \begin{minipage}{3.2cm}%5.5
    \includegraphics[width=17.2cm]{figures/legend}
   \end{minipage}
   \\
  \begin{minipage}{4.0cm}%5.5
    \includegraphics[width=4.3cm]{figures/hr_noise}
    \end{minipage}
    &
    \begin{minipage}{4cm}
    \includegraphics[width=4.3cm]{figures/mr_noise}
    \end{minipage}
    &
    \begin{minipage}{4cm}
    \includegraphics[width=4.3cm]{figures/hr_drop}
    \end{minipage}
    &
    \begin{minipage}{4cm}
    \includegraphics[width=4.3cm]{figures/mr_drop}
    \end{minipage}
    \\
    (a) Varying noise rate (HR@10)\hspace{-4mm}
    &
    (b) Varying noise rate (MRR)\hspace{-4mm}
    &
    (c) Varying drop rate (HR@10)\hspace{-4mm}
    &
    (d) Varying drop rate (MRR)\hspace{-4mm}
  % \begin{minipage}{0.43\linewidth}
	% \includegraphics[width=\linewidth]{figures/hr_noise}
  % \end{minipage}
  % &
  % \begin{minipage}{0.43\linewidth}
  %   \includegraphics[width=\linewidth]{figures/mr_noise}
  % \end{minipage}
  % \begin{minipage}{0.43\linewidth}
	% \includegraphics[width=\linewidth]{figures/hr_drop}
  % \end{minipage}
  % &
  % \begin{minipage}{0.43\linewidth}
  %   \includegraphics[width=\linewidth]{figures/mr_drop}
  % \end{minipage}
  % \\
  % (a) Varying noise rate (HR@10)
  % &
  % (b) Varying noise rate (MRR)
  % \\
  % \begin{minipage}{0.43\linewidth}
	% \includegraphics[width=\linewidth]{figures/hr_drop}
  % \end{minipage}
  % &
  % \begin{minipage}{0.43\linewidth}
  %   \includegraphics[width=\linewidth]{figures/mr_drop}
  % \end{minipage}
  % \\
  % (c) Varying drop rate (HR@10)
  % &
  % (d) Varying drop rate (MRR)
\end{tabular}
\vspace{-2mm}
%\setlength{\abovecaptionskip}{1pt}

\caption{Effectiveness with similarity search.}
\label{fig:effectiveness}
\vspace*{-2mm}
\end{figure*}
\fi

\begin{table}[]
\centering
{\extension{\caption {Effectiveness with classification and clustering.}}}\label{tab:tasks}
\vspace*{-3mm}
%\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|c|l|l|l|c|lcl}
\hline
\multirow{2}{*}{Tasks} & \multicolumn{4}{c|}{Classification} & \multicolumn{4}{c}{Clustering}                     \\ \cline{2-9}
                       & \multicolumn{4}{c|}{Acc (\%)}       & \multicolumn{2}{c}{ARI (\%)} & \multicolumn{2}{c}{AMI (\%)} \\ \hline
EMD                    & \multicolumn{4}{c|}{66.33}               & \multicolumn{2}{c}{52.15}    & \multicolumn{2}{c}{55.81}    \\
Hausdorff              & \multicolumn{4}{c|}{59.17}               & \multicolumn{2}{c}{51.68}    & \multicolumn{2}{c}{54.98}    \\
DTW                    & \multicolumn{4}{c|}{59.33}               & \multicolumn{2}{c}{50.12}    & \multicolumn{2}{c}{50.13}    \\
Frechet                & \multicolumn{4}{c|}{59.16}               & \multicolumn{2}{c}{50.16}    & \multicolumn{2}{c}{50.22}    \\
PM                        & \multicolumn{4}{c|}{54.24}               & \multicolumn{2}{c}{50.02}    & \multicolumn{2}{c}{50.32}    \\
DeepSets               & \multicolumn{4}{c|}{54.23}               & \multicolumn{2}{c}{49.50}    & \multicolumn{2}{c}{50.41}    \\
RepSet                 & \multicolumn{4}{c|}{58.99}               & \multicolumn{2}{c}{50.54}    & \multicolumn{2}{c}{50.72}    \\
WSSET                  & \multicolumn{4}{c|}{56.62}               & \multicolumn{2}{c}{49.12}    & \multicolumn{2}{c}{49.78}    \\
BL2Vec                 & \multicolumn{4}{c|}{\textbf{72.62}}               & \multicolumn{2}{c}{\textbf{61.94}}    & \multicolumn{2}{c}{\textbf{63.26}}    \\ \hline
\end{tabular}
\vspace*{-4mm}
\end{table}

\subsubsection{Experimental Results}
\label{sec:effectiveness}

\noindent \textbf{(1) Effectiveness evaluation (similarity search).}
The lack of ground truth makes it a challenging problem to evaluate the similarity. To overcome this problem, we follow recent studies~\cite{Arsomngern2021self} which propose to use the $HR@10$ and $MRR$ to quantify the similarity evaluation via self-similarity comparison. Specifically, we randomly select 100 billiards layouts to form the query set (denoted as $Q$) and 500 billiards layouts as the target database (denoted as $D$), For each billiards layout $ \mathcal{B}_q \in Q$, we create its positive version denoted as $\mathcal{B}_+$ by introducing two types of noises. As discussed in Section~\ref{subsec:sample}, (1) we shift each ball along a random direction by a random distance, which is controlled by a noise rate; (2) we randomly delete some balls controlled by a drop rate and then add them at random locations. Then for each $\mathcal{B}_q$, we compute the rank of $\mathcal{B}_+$ in the database $D \cup \mathcal{B}_+$ using BL2Vec and other baselines. Ideally, $\mathcal{B}_+$ should be ranked at the top since $\mathcal{B}_+$ is generated from the $\mathcal{B}_q$.



Figure~\ref{fig:effectiveness_similarity} (a) and (b) show the results of varying the noise rate from 0.2 to 0.4 when the drop rate is fixed to 0.2 in terms of
$HR@10$ and $MRR$. We can see that $BL2Vec$ is significantly better than the baselines in terms of $HR@10$ and $MRR$. For example, when applying 40\% noise, BL2Vec outperforms RepSet and DTW (the two best baselines) by 1.5 times and 4.7 times in terms of $HR@10$, respectively, and by more than 6.2 times and 13.3 times in terms of $MRR$, respectively. EMD and DeepSets perform the worst in most of the cases because EMD is based on the idea of point-matching and affected significantly by the noise;
DeepSets is developed for a set that has an unordered nature and therefore it is not suitable for measuring the similarity among billiards layouts, which are order sensitive. %In addition, compared with baselines, our BL2Vec is more robust to noise. For example, when the noise rate increases from 0.2 to 0.4, the $HR@10$ of BL2Vec only decreases by 15\%, while the values of DTW decrease by 80\%.
Figure \ref{fig:effectiveness_similarity} (c) and (d) show the results of varying the drop rate from 0.2 to 0.4 when the noise rate is fixed to 0.2 in terms of
$HR@10$ and $MRR$. BL2Vec still performs the best in terms of both metrics. For example, it outperforms RepSet, which performs best in baselines when the drop rate is 0.4, by more than 1.8 times and 9.6 times in terms of $HR@10$ and $MRR$. %We also note that the performance of BL2Vec gets worse with a larger drop rate. This is because the drop rate may change the form of their relative locations, which affects the similarity.

\noindent \textbf{(2) Effectiveness evaluation (classification).}
Table \ref{tab:tasks} shows the results of different methods in the classification task for predicting the labels of ``clear" and ``not clear". Recall that ``clear" means the player who performs the break shot pocketed all balls and thus win the game, and ``not clear" means the otherwise case.
%
We train a k-nearest neighbour classifier (kNN) with $k = 10$ for this task and report the average accuracy on 500 billiards layouts. For BL2Vec, we fix the noise rate and drop rate to be 0.2 by default, and use the representations of billiards layouts for computing the distance in the KNN classifier, we do the same for DeepSets, RepSet and WSSET. For EMD, Hausdorff, DTW, Frechet and PM, we use their distances for the KNN classifier directly.
We observe BL2Vec outperforms all the baselines. For example, it outperforms EMD (the best baseline) by 9.5\%. The result indicates that the representation learned from BL2Vec is more useful for learning the target task.

\noindent \textbf{(3) Effectiveness evaluation (clustering).}
We further show the clustering task, which is to group billiards layouts belonging to the same family (i.e., ``clear" or ``not clear") into the same cluster. We use the K-means algorithm with $k = 2$ and report ARI and AMI on the
500 billiards layouts. The results are shown in Table~\ref{tab:tasks}. According to the results, BL2Vec also performs best.
For example, it outperforms EMD (the best baseline) by 18.8\% (resp. 13.3\%) in terms of ARI (resp. AMI). In addition, we observe other baselines have similar ARI and AMI, e.g., the values are between 49\% and 50\%. Similar to the classification task, the results indicate adopting the embeddings of BL2Vec for billiards layout clustering will yield superior performance.

\noindent \textbf{(4) Effectiveness evaluation (parameter study).}
\label{sec:parameter}
We next evaluate the effect of the cell size on the effectiveness of similarity search, classification and clustering for BL2Vec.
Intuitively with the smaller cell size, it generates more tokens and provides a higher resolution of the pool table. However, with the smaller size, it reduces the robustness against the noise for the similarity search task. In Table \ref{tab:parameter}, we report the performance for the similarity search, classification and clustering. We notice that the performance of the similarity search becomes better as the cell size grows and this is in line with our intuition. In addition, we observe the smallest cell size of 10 leads to the worst performance, especially for classification and clustering, because the smallest cell size produces more tokens, which makes the model more difficult to train. In our experiments, we set the cell size to 15 because it provides better performance in general.

\begin{table}[]
\centering
{\extension{\caption {The effect of the cell size.}}}\label{tab:parameter}
%\vspace*{-2mm}
\centering
\setlength{\tabcolsep}{1.8pt}
\begin{tabular}{c|c|cc|c|l|l|l|c|lcl}
\hline
\multirow{2}{*}{Cell size} & \multirow{2}{*}{\#tokens} & \multicolumn{2}{c|}{Similarity} & \multicolumn{4}{c|}{Classification} & \multicolumn{4}{c}{Clustering}                     \\ \cline{3-12}
                           &                           & HR@10           & MRR           & \multicolumn{4}{c|}{Acc (\%)}       & \multicolumn{2}{c}{ARI (\%)} & \multicolumn{2}{c}{AMI (\%)} \\ \hline
10                         &    200                    &  0.92         & 0.240              & \multicolumn{4}{c|}{66.67}               & \multicolumn{2}{c}{52.25}    & \multicolumn{2}{c}{55.80}    \\
15                         &    98                     &  0.94         & 0.252         & \multicolumn{4}{c|}{\textbf{72.62}}               & \multicolumn{2}{c}{\textbf{61.94}}    & \multicolumn{2}{c}{\textbf{63.26}}    \\
20                         &    50                     & 0.95          &0.259          & \multicolumn{4}{c|}{67.33}               & \multicolumn{2}{c}{56.96}    & \multicolumn{2}{c}{58.25}    \\
25                         &    32                     &  0.96          &0.303              & \multicolumn{4}{c|}{70.14}               & \multicolumn{2}{c}{55.21}    & \multicolumn{2}{c}{57.37}    \\
30                         &    28                     &  \textbf{0.96}          &\textbf{0.306}            & \multicolumn{4}{c|}{68.72}               & \multicolumn{2}{c}{53.96}    & \multicolumn{2}{c}{56.28}    \\ \hline

\end{tabular}
%\vspace*{-3mm}
\end{table}

\begin{table}[]
\centering
{\extension{\caption {Effectiveness evaluation with ablation study.}}}\label{tab:ablation}
%\vspace*{-3mm}
%\footnotesize{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{c|cc|c|l|l|l|c|lcl}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{Similarity} & \multicolumn{4}{c|}{Classification} & \multicolumn{4}{c}{Clustering}                     \\ \cline{2-11}
                       & HR@10           & MRR           & \multicolumn{4}{c|}{Acc (\%)}       & \multicolumn{2}{c}{ARI (\%)} & \multicolumn{2}{c}{AMI (\%)} \\ \hline
BL2Vec                 & \textbf{0.94}            & \textbf{0.252}              & \multicolumn{4}{c|}{\textbf{72.62}}               & \multicolumn{2}{c}{\textbf{61.94}}    & \multicolumn{2}{c}{\textbf{63.26}}    \\
w/o BS                 & 0.92            & 0.207              & \multicolumn{4}{c|}{62.42}               & \multicolumn{2}{c}{53.50}    & \multicolumn{2}{c}{59.25}    \\
w/o BP                 & 0.11            & 0.009              & \multicolumn{4}{c|}{51.08}               & \multicolumn{2}{c}{49.27}    & \multicolumn{2}{c}{50.18}    \\
w/o BB                 & 0.91            & 0.197              & \multicolumn{4}{c|}{69.52}               & \multicolumn{2}{c}{52.45}    & \multicolumn{2}{c}{61.73}    \\ 
w/o $Net(\cdot)$       &  0.40          & 0.078             & \multicolumn{4}{c|}{41.76}               & \multicolumn{2}{c}{50.38}    & \multicolumn{2}{c}{50.67}   \\ \hline
\end{tabular}%}
%\vspace*{-3mm}
\end{table}

\noindent \textbf{(5) Effectiveness evaluation (ablation study).}
\label{sec:ablation}
To show the importance of each component of the extracted features in our BL2Vec model, including Ball-self (BS), Ball-Pocket (BP) and Ball-Ball (BB), and the ability of CNN for capturing spatial features in $Net(\cdot)$, we conduct an ablation experiment. We denote our BL2Vec model without BS, BP, BB and $Net(\cdot)$ as w/o BS, w/o BP, w/o BB and w/o $Net(\cdot)$, respectively. Table~\ref{tab:ablation} compares the different versions for similarity search, classification and clustering tasks. Overall, all these components help improve the effectiveness of the BL2Vec model and enable the model to achieve superior performance than baselines. A detailed discussion on the effectiveness of each component is given as follows.
%
(1) BS features can effectively capture the spatial information of each ball; if the features are omitted, the classification performance drops significantly by around 14\%. %{\color{blue}
(2) BP features capture the correlations between the ball and each pocket, and these are the unique characteristics in the billiards layout data. In addition, BP features are associated with the most tokens (i.e., $4 \times 6 =24$) in the total of 27 tokens to represent each ball as discussed in Section~\ref{subsec:feature_extraction}, and therefore the BP features contribute the most for all of the tasks. As expected, we observe that if the BP features are omitted, the performance of similarity search drops by 88\% (resp. 96\%) in terms of HR@10 (resp. MRR); that of classification drops by 30\% in terms of accuracy; that of clustering drops by 20\% (resp. 21\%) in terms of ARI (resp. AMI). (3) BB features capture the correlation between balls in the layout. The features also affect the overall performance. For example, if the BB features are omitted, the clustering performance drops a lot by around 15\% (resp. 2\%) in terms of ARI (resp. AMI). (4) The CNN in $Net(\cdot)$ can well capture the correlation of those spatial features (i.e., BS, BP and BB), and simply using the average of feature embeddings cannot lead to the superior performance, e.g., similarity search drops by 57.4\% (resp. 69.05\%) in terms of HR@10 (resp. MRR).

% \begin{figure}
% \begin{tabular}{c c}
% \begin{minipage}{0.45\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figures/running_time}
% %\setlength{\abovecaptionskip}{1pt}
% %\vspace*{-4mm}
% \caption{{\nnComment{Scalability.}}}
% \label{fig:efficiency}
% \end{minipage}
% &
% \begin{minipage}{0.45\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figures/user_study}
% %\setlength{\abovecaptionskip}{0pt}
% %\vspace*{-4mm}
% \caption{User study.}
% \label{fig:userstudy}
% \end{minipage}
% \end{tabular}
% %\vspace*{-4mm}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/running_time}
% \caption{Scalability.}
% \label{fig:efficiency}
% \end{figure}

%\begin{figure}
%%\hspace*{-.3cm}
%\centering
%\begin{tabular}{c c}
%  \begin{minipage}{0.99\linewidth}
%	\includegraphics[width=\linewidth]{figures/running_time}
%  \end{minipage}
%\end{tabular}
%%\vspace{-2mm}
%%\setlength{\abovecaptionskip}{1pt}
%\caption{Efficiency evaluation.}
%\label{fig:efficiency}
%\end{figure}


% We also study our improvements on feature engineering of billiards layouts for the spatial data. Table \ref{tab:ablation} shows BL2Vec performance on three
% different conditions. Feature engineering of billiards layouts consists of three kinds of features. Firstly, we talk about BS features.
% It is positions of balls in each billiards layout, which are transformed into tokens by dividing cells on the pool table, which has been introduced in parameter study.
% From the table, we notice that if BS features are omitted, the performance of BL2Vec on accuracy and clustering are worse.
% We next talk about BP features. It is ball-to-pocket features. We know there are 6 pockets on the pool table. For each pocket, we use 4 features to
% represent features of the ball to it. These four features are a minimum value between the degree between the vector from the ball to the pocket and the eft cushion
% and the degree between the vector from the ball to the pocket and right cushion, the distance from a ball to a pocket, 0/1 to denote whether the pocket can be potted or not because
% if a ball whose number is larger than the ball lies in the path from the current ball with the smallest number on the billiards
% table to a pocket, we know the current ball cannot be potted to this pocket with the index is equal to 0, the index is equal to 1 otherwise, and the last feature is the pocket index from 0 to 5 namely 6 pockets on the pool table.
% Because there are 6 pockets on the poll table and the number of features from the current ball to each pocket are 4, there are 24 features represent the second kind of features belonging to BP (ball-to-pocket).
% From the table, we can notice that when these 24 features are omitted, the performance of BL2Vec in similarity, classification and clustering are worst, with HR@10 0.08, MRR 0.005, Accuracy 50.37, ARI 49.50 and AMI 49.65.
% The last kind of features are belonging to BB, which represents features from the former ball to the current ball. It consists of two features, namely the most possible pocket index which represents the most possible pocket the current ball can be potted and
% the degree between the vector from the former ball to the current ball and the vector from the current ball to the most possible pocket.
% We can see from the table that omitting this kind of features affects a little performance on similarity. Thus, we can see that BP features are the most important features for the BL2Vec.


\begin{figure}[ht]
%\footnotesize
%\vspace*{-1mm}
\centering
\begin{tabular}{c c}
%   \begin{minipage}{8.5cm}
%     \includegraphics[width=17.2cm]{figures/running_time_legend.pdf}
%   \end{minipage}
%   &
    \\
   \begin{minipage}{3.9cm}
    \includegraphics[width=4.1cm]{figures/embedding_time.pdf}
    \end{minipage}
    &
    \begin{minipage}{3.8cm}
    \includegraphics[width=4cm]{figures/running_time.pdf}
    \end{minipage}
    \\
    (a) Embedding scalability 
    &
    (b) Search scalability
\end{tabular}
\vspace*{-2mm}
{\extension{\caption{Scalability test.}}}
\vspace*{-2mm}
\label{fig:efficiency}
\end{figure}
\noindent \textbf{(6) Scalability test.}
\label{sec:efficiency}
%In this part, we evaluate the efficiency of different methods for the billiards layout retrieval over 100 queries. 
To test scalability, we generate more layouts by adding noise on the original dataset.
{\ICDEComment{Figure \ref{fig:efficiency}(a) reports the running time of embedding the database from 1 million layouts to 5 million layouts for the learning-based methods, i.e., DeepSets, WSSET, Rapset and BL2Vec.
}}
Figure \ref{fig:efficiency}(b) reports the average running time over 10 queries for computing the similarity between a query billiards layout and the billiards layouts when we vary the size of the target database from 1 million layouts to 5 million layouts. 
%

{\ICDEComment{For embedding time, we notice all learning-based methods have their running times linearly increase with the dataset size, which is consistent with their linear time complexity for embedding layouts. We observe DeepSets model is fastest for the embedding, because the model is light via embedding each point into a vector, and aggregating all embeddings together to an overall embedding of the pointsets, 
which can be accomplished very quickly. Overall, BL2Vec runs comparably fast for the layout embedding, compared with other learning-based  methods.
}}

For searching time, EMD and Hausdorff perform extremely slow, which match their quadratic time complexity.
%
We observe the running time of DTW and Frechet is smaller than that of EMD and Hausdorff though all of them have the same time complexity. This is because DTW and Frechet compute the similarity via dynamic programming to find an
optimal pairwise point-matching.
%
%{\color{blue}
PM is faster than DTW and Frechet because it matches the balls peer-to-peer based on their numbers and the complexity is linear.%}
In addition, DeepSets, WSSET, Rapset and BL2Vec have a similar running time.
Specifically, they run up to 420 times faster than EMD and Hausdorff, 160 times faster than DTW and Frechet and 100 times faster than PM. Moreover, we notice that DeepSets, WSSET, Rapset and BL2Vec scale linearly with the dataset size and the disparity between them increases as the size of the target database grows. This is because all of the learning-based methods have linear time complexity to compute the similarity by embedding layouts to vectors, and the embedding process can also be done offline, which is consistent with their time complexities.
%the discussion in Section~\ref{subsec:complexity}.

\begin{figure}
\centering
\begin{tabular}{c c}
   \begin{minipage}{3.9cm}
    \includegraphics[width=4.1cm]{figures/training_effectiveness.pdf}
    \end{minipage}
    &
    \begin{minipage}{3.9cm}
    \includegraphics[width=4.1cm]{figures/training_time.pdf}
    \end{minipage}
    \\
    (a) HR@10
    &
    (b) Time cost 
\end{tabular}
\vspace*{-2mm}
{\extension{\caption{Training cost.}}}
\label{fig:traing}
\vspace*{-2mm}
\end{figure}

\noindent \textbf{(7) Training time.}
\label{sec:training}
{\ICDEComment{The training time of BL2Vec is shown in Figure~\ref{fig:traing}. In particular, we study how the number of training samples affects the model performance for similarity search (i.e., $HR@10$) and the training time cost. We randomly 5 training sets from the dataset, including 500, 1,000, 1,500, 2,000, 2,500 billiards layouts, respectively. For each training set, we report
its training cost per epoch and the corresponding effectiveness on 
the testing set with 500 layouts, where we follow the default setup in Section~\ref{sec:setup}. 
%
Based on the results, we observe the effectiveness improves as the training size increases, and it approximately converges when the training size exceeds 2,000. For the training time, it increases almost linearly with the training size as expected. We use the setting of 70\% (i.e., 2,000) billiards layouts for training, since it provides a reasonable trade-off between effectiveness and training cost.}}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/user_study}
%\vspace*{-4mm}
{\extension{\caption{User study.}}}
\label{fig:userstudy}
%\vspace*{-4mm}
\end{figure}

\begin{figure*}
\centering
\begin{tabular}{c c c c c}
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/query_63_63}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_40_40}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/query_42_42}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_43_43}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_46_46}%
  \end{minipage}
  \\
  Q1
  &
  Q2
  &
  Q3
  &
  Q4
  &
  Q5
  \\
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dtw_63_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_40_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dtw_42_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_43_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_46_0}%
  \end{minipage}
  \\
  DTW 1 (1/10)
  &
  DTW 2 (2/10)
  &
  DTW 3 (1/10)
  &
  DTW 4 (6/10)
  &
  DTW 5 (6/10)
  \\
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dml_63_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_40_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dml_42_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_43_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_46_0}%
  \end{minipage}
  \\
  BL2Vec 1 (9/10)
  &
  BL2Vec 2 (8/10)
  &
  BL2Vec 3 (9/10)
  &
  BL2Vec 4 (4/10)
  &
  BL2Vec 5 (4/10)
\end{tabular}
%\vspace*{-3mm}
{\extension{\caption{Top-1 billiards layouts for Q1-Q5 returned by DTW and BL2Vec, (1/10) means the 1 user supports this result among the total of 10 users.}}}
%\vspace{-4mm}
\label{q1toq5}
%\vspace*{-4mm}
\end{figure*}

\begin{figure*}
\centering
\begin{tabular}{c c c c c}
 \begin{minipage}{0.18\linewidth}
 \includegraphics[width=\linewidth]{figures/user/query_50_50}%
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_16_16}%
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
 \includegraphics[width=\linewidth]{figures/user/query_82_82}%
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_78_78}%
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/query_84_84}%
 \end{minipage}
 \\
 Q6
 &
 Q7
 &
 Q8
 &
 Q9
 &
 Q10
 \\
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_50_0}%-eps-converted-to
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
 \includegraphics[width=\linewidth]{figures/user/dtw_16_0}%-eps-converted-to
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_82_0}%-eps-converted-to
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
 \includegraphics[width=\linewidth]{figures/user/dtw_78_0}%-eps-converted-to
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_84_0}%-eps-converted-to
 \end{minipage}
 \\
 DTW 6 (0/10)
 &
 DTW 7 (1/10)
 &
 DTW 8 (1/10)
 &
 DTW 9 (1/10)
 &
 DTW 10 (0/10)
 \\
 \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_50_0}%-eps-converted-to
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
 \includegraphics[width=\linewidth]{figures/user/dml_16_0}%-eps-converted-to
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_82_0}%-eps-converted-to
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
 \includegraphics[width=\linewidth]{figures/user/dml_78_0}%-eps-converted-to
 \end{minipage}
 &
 \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_84_0}%-eps-converted-to
 \end{minipage}
 \\
 BL2Vec 6 (10/10)
 &
 BL2Vec 7 (9/10)
 &
 BL2Vec 8 (9/10)
 &
 BL2Vec 9 (9/10)
 &
 BL2Vec 10 (10/10)
\end{tabular}
%\vspace*{-3mm}
{\extension{\caption{Top-1 billiards layouts for Q6-Q10 returned by DTW and BL2Vec.}}}
\label{q6toq10}
%\vspace*{-4mm}
\end{figure*}

\begin{figure*}
\centering
\begin{tabular}{c c c c c}
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dtw_63_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_63_1}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dtw_63_2}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_63_3}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dtw_63_4}%
  \end{minipage}
  \\
  DTW 1 (1/10)
  &
  DTW 2
  &
  DTW 3
  &
  DTW 4
  &
  DTW 5
  \\
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dml_63_0}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_63_1}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
  \includegraphics[width=\linewidth]{figures/user/dml_63_2}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_63_3}%
  \end{minipage}
  &
  \begin{minipage}{0.18\linewidth}
    \includegraphics[width=\linewidth]{figures/user/dml_63_4}%
  \end{minipage}
  \\
  BL2Vec 1 (9/10)
  &
  BL2Vec 2
  &
  BL2Vec 3
  &
  BL2Vec 4
  &
  BL2Vec 5
  \\
\end{tabular}
%\vspace*{-2mm}
{\extension{\caption{Top-5 billiards layouts for Q1 returned by the DTW and BL2Vec (from left to right).}}}
%\vspace*{-4mm}
\label{top5}
\end{figure*}

\noindent \textbf{(8) User study.}
Since DTW performs the best among all baselines in the similar billiards layout retrieval task as shown in Figure~\ref{fig:effectiveness_similarity}, we conduct a user study to compare the BL2Vec with DTW. We randomly select 10 billiards layouts as the query set as shown in the first row in Figure~\ref{q1toq5} and Figure~\ref{q6toq10}, and for each query in the query set, we use BL2Vec and DTW to retrieve Top-1 billiards layouts from the target database. 
%
We invite ten volunteers with strong billiards knowledge to annotate the relevance of the retrieved results. More specifically, we firstly spent 15 minutes on introducing the background to the volunteers so that they understand these images as shown in Figure~\ref{q1toq5} and Figure~\ref{q6toq10}. Then for each of 10 queries, the volunteers specify the more similar result from the Top-1 result retrieved by BL2Vec and the Top-1 result retrieved by DTW. Note that the volunteers do not know which result is returned by which method in advance. We report the scores of the ten queries for both methods in Figure~\ref{fig:userstudy}. We observe that our BL2Vec outperforms DTW with expert knowledge. In particular, BL2Vec outperforms DTW for 8 queries out of the total 10 queries. In addition, BL2Vec gets 81\% votes while DTW gets only 19\% votes. We illustrate the Top-1 results of BL2Vec and DTW for Q1 to Q5 and Q6 to Q10 in Figure~\ref{q1toq5} and Figure~\ref{q6toq10}, respectively. From these figures, we observe the layouts retrieved by BL2Vec match the queries very well. For example, we find that the overall layout of the TOP-1 result by BL2Vec is very similar to Q1. %%and Top 2-5 results also maintain high consistency in the layouts. %{\color{blue}
DTW is slightly better than BL2Vec for Q4 and Q5 (i.e., 2\% votes). This is because the overall layouts returned by DTW are more similar to the queries; however, DTW falsely matches the balls, e.g., 9 balls in Q4, but the layout returned by DTW only has 7 balls and they are matched with different colors. It indicates that the pairwise point-matching solution is not suitable for the billiards layout retrieval task. {\ICDEComment{In addition, we visualize the Top 5 results for Q1 returned by the DTW and BL2Vec in Figure~\ref{top5}, we observe BL2Vec maintains a high consistency between the retrieved Top 2-5 results and the query.
% , and outperforms the DTW based on the visual.
}}



==> introduction.tex <==

\section{INTRODUCTION}
\label{sec:introduction}

% Nowadays, it becomes a common practice to collect data about sports with different tools such as GPS devices and cameras.
% The collected data precipitates research in many analytics tasks such as 
Recently, many studies of mining sports data are emerging, including
similar play retrieval~\cite{sha2016chalkboarding,wang2019effective}, tactics discovery~\cite{decroos2018automatic}, sports video detection~\cite{liu2005effective}, team formation detection~\cite{bialkowski2014large,lucey2013representing}, sports pattern mining~\cite{decroos2018automatic,miller2014factorized}, score prediction~\cite{aoki2017luck,yue2014learning}, 
% and {\color{blue}
activity recognition~\cite{brunner2019swimming,cuspinera2016beach,bachlin2009swimmaster}, etc.
These studies cover various sports domains, including basketball, soccer, volleyball and swimming. 
%
{\ChengComment{Yet this data-driven approach remains largely unexplored on billiards.
% which is one type of popular sports.
Billiards is a sports game where players play with a cue stick on a billiards table with six pockets. 
In a billiards game, players strike the cue (white) ball to an object (coloured) ball, with the intent to drive the object ball into a pocket. 
%Popular billiards games include 9-ball, 8-ball and Snooker.
}}

In this paper, we expand this line of research to billiards sports. 
% Billiards is a popular sports, where players strike the cue (white) ball to an object (colored) ball, with the intent to drive the object ball into a pocket. Popular billiards games include 9-ball, 8-ball and Snooker.
% Based on the collected dataset, we propose to study the \emph{similar billiards layout retrieval} (or simply similar layout retrieval) problem, which aims to find those billiards layouts from a database that are similar to a query billiards layout called \emph{query layout}.
Specifically, we study the \emph{similar billiards layout retrieval} (or simply similar layout retrieval) problem, which is to find those billiards layouts from a database that are similar to a billiards layout at hand called \emph{query layout}. 
Here, a billiards layout consists of the locations and identities of the balls (including the cue ball and the object balls) after a strike during a game. 
{\ChengComment{Figure~\ref{fig:example_intro} shows an example of a 9-ball billiards layout.}}
Intuitively, a billiards layout embeds rich information of a game that could help to inform many aspects of the game, e.g., what's the winning probability of a player, what's the strategy to strike the balls, and is there any historical layout that can be used as a reference point, etc.

\begin{figure}
\vspace*{-2mm}
\centering
\begin{tabular}{c}
  \begin{minipage}{0.8\linewidth}
	\includegraphics[width=\linewidth]{figures/data_example2.pdf}
  \end{minipage}
\end{tabular}
\vspace*{-2mm}
\caption{A real 9-ball billiards layout.}
\vspace*{-3mm}
\label{fig:example_intro}
\end{figure}

The similar layout retrieval problem can be used in many scenarios. One scenario is to provide a real-time prediction of the winning result of a game given the latest layout, for which one intuitive solution is to make similar predictions for games with \emph{similar} layouts. This prediction functionality is highly desirable by Web broadcasting platforms of the billiards games such as %{\color{red}
ChalkySticks~\footnote{https://www.chalkysticks.com/tv}. Another scenario is that a billiards coach would like to analyze how well a player performs given different layouts after the first strike (called the break shot). In this scenario, the coach can retrieve those historical layouts that are \emph{similar} to a given one and their performance results (e.g., winning or not) and collect some statistics based on the retrieved layouts. This application can be implemented as a web-based searching engine, putting all layouts at a web server and providing a search functionality to coaches to look for similar layouts for training. A third scenario could be that a billiards fan is watching a billiards game during which, he/she finds some layouts interesting and would like to find if there are \emph{similar} layouts and/or games in the past - note that a game corresponds to a sequence of layouts and if so, how the players play given those layouts. %}

\if 0
Billiards layout retrieval is a fundamental research problem and is a foundation for many emerging applications, and we now discuss the applications as follows.
%such as recommending billiards games to sports fans by finding a game based on searching two games with the layout after the break shot similar to a query one. Besides, it could help players to improve his strategy and physical skills by training on some similar layouts~\cite{archibald2009analysis,smith2006running}.
{\color{blue}
\begin{itemize}
\item Sports recommendation. It becomes very common in some sports applications such as ESPN~\footnote{https://www.espn.com} to recommend similar sports games to users when they browse a game. Suppose that ESPN wishes to recommend a billiards game, denoted by $G$, to a billiards fan when he watches a billiards game $G_q$. A straightforward solution is to somehow align the two games, i.e., $G_q$ and $G$, and measure the similarity between each layout in $G_q$ and the corresponding layout in $G$, then the overall similarity of the two games is defined by aggregating the similarities of all layouts in the game. In this scenario, the layout similarity computation is a building block to support the recommendation task. Also, these applications often have to handle the recommendation for a large number of online users. A high-performance similarity measurement can therefore benefit these applications.
\item Game strategy training. A common application scenario for billiards layout retrieval is to specify some similar layouts for players to improve their strategy and physical skills. For example, the break shot is a crucial shot that affects the outcome of a billiards game. Billiards layout retrieval allows players training his strategies under some certain types of break shot layouts when he prepares an upcoming game.
\item Data analysis. A common data analysis task is to conduct the classification. For example, based on the break shot layouts, some mobile apps may be proliferated to provide instant feedback on the break performance for players, e.g., taking a picture of a break shot layout and import the picture into a mobile app to infer the quality or the likelihood for the player to clear the table and thus win the frame. In this paper, we study the classification task by training a k-nearest neighbor classifier based on the billiards layout similarity.
\end{itemize}
}
\fi

The core challenge of similar billiards layout retrieval is that of measuring the similarity between two billiards layouts, which is non-trivial due to some unique characteristics of billiards layouts.
% since billiards layouts contain some characteristics that make them unique among existing similarity measurements.
First, billiards layouts are order sensitive, e.g., in a billiards 9-ball game, the object balls are numbered from 1 to 9 and players should legally strike the object ball numbered the lowest in the layout first.
Therefore, existing similarity measures on sets (or pointsets), which include (1) pairwise point-matching such as Earth Mover's Distance (EMD)~\cite{rubner2000earth} and Hausdorff distance~\cite{huttenlocher1993comparing} and (2) recently emerging learning-based techniques such as DeepSets~\cite{zaheer2017deep} and RepSet~\cite{skianis2020rep}, all assume order invariance and thus they are not suitable for billiards layouts. 
% In particular, those measures based on (1) pairwise point-matching such as Earth Mover's Distance (EMD)~\cite{rubner2000earth} or Hausdorff distance~\cite{huttenlocher1993comparing}, and (2) recently emerging learning-based techniques such as DeepSets~\cite{zaheer2017deep} or RepSet~\cite{skianis2020rep} all compute the similarity to be invariant in the order of the points in a set.
% Indeed, some measures can treat the unordered sets as ordered sequences, and compute the similarity by identifying the best alignment via dynamic programmings, such as
{\ChengComment{We note that existing similarity measures on sequences and trajectories such as DTW~\cite{yi1998efficient}, Frechet~\cite{alt1995computing},
LCSS~\cite{vlachos2002discovering}, ERP~\cite{chen2004marriage}, EDR~\cite{chen2005robust}, and EDwP~\cite{ranu2015indexing}}}, though order sensitive, are not suitable for billiards layouts either. This is because they would align the balls from two layouts solely based on their locations and totally ignore other information such as the ball numbers.
{\ChengComment{For example, for two billiards layouts with totally different object balls such as Figure~\ref{fig:problem} (c) and (d), it is counter-intuitive to align these different coloured balls to compute the similarity.}}
%
Second, billiards layout data is with some domain-specific features, e.g., the types and locations of pockets, the factors deciding the difficulty of striking an object ball to a pocket such as the angle formed by the cue ball, a target object ball and a pocket, etc. These features are important for measuring similarities among billiards layouts and should be systematically captured in the similarities.
% e.g., the spatial correlation of balls and/or pockets in the layout, and it remains unexplored to capture them in a similarity measure.
% Thus, a good similarity measure needs to take these features into consideration; however, existing measures fail to capture the similarity in this aspect.


{\nnComment{Another challenge is efficiency. A typical application scenario of similar billiards layout retrieval is to compute the similarity between a query billiards layout and many billiards layouts in the database. However, the existing matching-based methods all involve the procedure of finding an optimal alignment~\cite{yi1998efficient,alt1995computing}, which has at least a quadratic time complexity in terms of the number of balls and would impose a big challenge when performing similar layout retrieval on a huge database}} {\ChengComment{with many layouts and for a big number of queries since the operation of computing the similarity between two layouts needs to be conducted for many pairs of data layouts and query layouts.}}

In this paper, we propose a novel solution called BL2Vec, which overcomes the aforementioned challenges of similar billiards layout retrieval. Regarding the effectiveness, we leverage a deep metric learning model, namely \emph{triplet network}~\cite{kaya2019deep}, to learn a ranking-based metric for measuring the similarities among billiards layouts. More specifically, to capture the ordered nature of the billiards layout data, we treat billiards layouts as ordered sequences, i.e., one cue ball followed by several object balls in the ascending order of their numbers and apply padding when there are missing balls (since some may have been pocketed). To capture those unique characteristics in billiards layouts, we propose to extract features from the balls and pockets and further embed them. Then, we use Convolutional Neural Network (CNN)~\cite{lecun1998gradient} to generate a vector from the embedded features as the representation of the layout since CNN can inherently capture the local relationships between the balls. In addition, we propose a method to generate training data with hard negative mining~\cite{henriques2013beyond} so that BL2Vec is robust to a small shift in a billiards layout and learns the similarity in a self-supervised manner. 
% BL2Vec significantly differs from the existing measures that capture the similarity with some hand-crafted rules/objectives such as pairwise point-matching.
%
{\nnComment{Regarding the efficiency, our method based on BL2Vec computes the similarity between two layouts as the Euclidean distance between their representations (i.e., vectors), which runs in linear time wrt the number of balls in a game.}} 
% existing methods that involve pairwise point-matching have time complexities at least $O(n^2)$, where $n$ denotes the number of balls in the layout. 
When performing a similar layout retrieval on a database, we first learn the representations of billiards layouts once offline. Then, for a given query layout, we learn its representation and perform a \emph{nearest neighbour} query in the representation space (i.e., the vector space), which could be efficiently accomplished with existing methods such as the one in~\cite{bentley1975multidimensional}.
% locality-sensitive hashing~\cite{indyk1998approximate}.
% After embedding the billiards layouts into vectors offline, the similarity between two layouts is captured by the Euclidean distance, which could be computed in constant time and therefore the complexity of searching a billiards layout is linear with the size of the database. The linear complexity makes BL2Vec suitable for large datasets.

Given that there are no billiards layout datasets that are publicly available, we further collect a billiards layout dataset.
% , which will be made publicly available.
%
%layout
% A billiards layout corresponds to a set of billiards balls including a cue ball and several object balls, which are located on a billiards table.
% {\ChengComment{Figure~\ref{fig:example_intro} shows an example of a 9-ball billiards layout.}}
%
In particular, the dataset consists of 3,019 billiards (9-ball) layouts after break shots~\footnote{https://en.wikipedia.org/wiki/Glossary\_of\_cue\_sports\_terms}, and covers international professional billiard tournaments including China Open, All Japan and 9-Ball World Championships~\footnote{https://wpapool.com/ranking/} in the last two decades.
The dataset was collected with a free sports analysis software Kinovea~\footnote{http://www.kinovea.org} and contains rich remarks (e.g., golden break or foul) and labels including \emph{the number of potted balls} after the break shot, \emph{clear or not} and \emph{win or not} based on the layout. 
This dataset would provide opportunities of conducting various billiards-related analytics tasks.

In summary, the paper makes the following contributions: 
% (1) We propose the similar billiards layout retrieval problem and a deep learning-based similarity measure called BL2Vec for billiards layouts. To the best of our knowledge, {\nnComment{this is the first work on billiards layout similarity, and BL2Vec is the first deep learning-based solution.}} %for learning similarity between billiards layouts. 
% The similarity not only considers the unique characteristics in a billiards layout but also runs fast. (2) We conduct extensive experiments on the collected 9-ball data, which demonstrate that our method consistently outperforms the baseline methods for measuring billiards layout similarity. The efficiency experiments show that our method runs up to $420 \times$ faster than the existing methods that involve pairwise point-matching for measuring the similarity between two layouts. We further conduct a user study, which validates our method with expert knowledge. Our collected dataset and codes will be made publicly available.
\begin{enumerate}[leftmargin=*]
    
    
    \item We propose the similar billiards layout retrieval problem and a deep learning-based similarity measure called BL2Vec for billiards layouts. To the best of our knowledge, BL2Vec is the first deep learning-based solution for learning similarity between billiards layouts. The similarity not only considers the unique characteristics in a billiards layout but also runs fast in linear time.
    
    % \item We collect a billiards layout dataset. The data covers international professional billiard matches in the most recent two decades. It also has rich remarks and labels information to support various billiards-related analytics tasks. To the best of our knowledge, it would be the first publicly available dataset of billiards layouts.
    
    \item We conduct extensive experiments on the collected 9-ball data, which demonstrate that our method consistently outperforms the baseline methods for measuring billiards layout similarity. {\ICDEComment{The effectiveness experiments show that our method can outperform the best baseline by at least 27\% for similarity search.}}
    The efficiency results show that our method runs up to $420 \times$ faster than the existing methods that involve pairwise point-matching for measuring the similarity between two layouts. We further conduct a user study, which validates our method with expert knowledge.
    
    \item {\newadd{Our collected dataset and codes could be accessed via this link~\footnote{\url{https://www.dropbox.com/sh/644aceaolfv4rky/AAAKhpY1yzrbq9-uo4Df3N0Oa?dl=0}}.}}
\end{enumerate}
%via the link~\footnote{https://www.dropbox.com/sh/uzszs259ggmyntz/AAAM0zh\_TKmkfdJNaEdCD3cRa?dl=0}
%We will publish the dataset once the paper is accepted, which 
% will be made publicly available.

The rest of the paper is organized as follows. We review the literature in Section~\ref{sec:related} and give the problem definition in Section~\ref{sec:problem}. We present our BL2Vec model in Section~\ref{sec:method}, {\ChengComment{the dataset in Section~\ref{sec:dataset}}}, and report our experimental results in Section~\ref{sec:experiment}. We finally conclude the paper and discuss some future work in section~\ref{sec:conclusion}.


==> problem.tex <==
{\extension{
\section{PROBLEM DEFINITION}
\label{sec:problem}

% \subsection{Background of Billiards Game}
% \label{subsec:background}
%We provide a brief background for readers to easily understand some unique characteristics of the billiards layout data.
%
A billiards game refers to a game playing with a cue stick on a rectangular billiards table, which has six pockets at the four corners and in the middle of each long side. The game involves a cue ball (white) and some object balls (colored), where different billiards games have different numbers of object balls such as 9 object balls in 9-ball game. %, 15 object balls in 8-ball game and 21 object balls in Snooker game.
%
The game begins with one player's break shot. If a ball is legally pocketed after the break shot, the player keeps his turn; otherwise, the opponent gets a chance to shoot.
%
% The legally pocketed are constrained by the order of balls in the layout,
% The game begins with one player's break shot. 
%Players should obey some rules when playing the game, e.g, a player must strike the cue ball to pocket nine colored balls in an ascending order of their numbers in the 9-ball game, in the way the player can retain his turn; otherwise, the opponent gets a chance to shoot.
% The legally pocketed determines some rules in a game, 
There are usually some rules to follow when striking a ball,
e.g, in a 9-ball game, a player must use the cue ball (white) to strike the object balls (colored) in an ascending order of their numbers.
% %
%The player can retain his turn as long as he calls an object ball legally and make the called ball sink into a pocket.
%
%In case of an illegal shot (i.e., foul), such as sinking the cue ball into a pocket, it offers the opponent "ball in hand", which means the cue ball can be placed at any location on the table.



% \subsection{Problem Definition}
% \begin{figure*}
% %\hspace*{-.3cm}
% \centering
% \begin{tabular}{c c c c}
%   \begin{minipage}{0.22\linewidth}
% 	\includegraphics[width=\linewidth]{figures/problem1}
%   \end{minipage}
%   &
%   \begin{minipage}{0.22\linewidth}
%     \includegraphics[width=\linewidth]{figures/problem2}
%   \end{minipage}
%   &
%   \begin{minipage}{0.22\linewidth}
% 	\includegraphics[width=\linewidth]{figures/problem3}
%   \end{minipage}
%   &
%   \begin{minipage}{0.22\linewidth}
%     \includegraphics[width=\linewidth]{figures/problem4}
%   \end{minipage}
%   \\\\
%   (a) \footnotesize{$\mathcal{B}_q$ (cue ball and ball 2,7,9)}
%   &
%   (b) \footnotesize{$\mathcal{B}_1$ (cue ball and ball 2,7,9)}
%   &
%   (c) \footnotesize{$\mathcal{B}_2$ (cue ball and ball 2,7,9)}
%   &
%   (d) \footnotesize{$\mathcal{B}_3$ (cue ball and ball 3,4,6)}
% \end{tabular}
% %\vspace{-2mm}
% %\setlength{\abovecaptionskip}{1pt}
% \caption{An example of illustrating the billiards layout similarity, where $sim(\mathcal{B}_q, \mathcal{B}_1) > sim(\mathcal{B}_q, \mathcal{B}_2) > sim(\mathcal{B}_q, \mathcal{B}_3)$.}
% \label{fig:problem}
% \vspace*{-5mm}
% \end{figure*}

%\begin{table}
%	\centering
%		%  \setlength{\abovecaptionskip}{1pt}
%		\setlength{\belowcaptionskip}{0pt}
%		\caption {Notations for billiards layout similarity.}\label{notation}
%		\begin{tabular}{c|c}
%			\hline
%			{\bf Notation}     & {\bf Meaning}\\
%			\hline\hline
%			%          $T$          & trajectory\\
%			$\mathcal{D}$  & database of billiards layouts\\
%			\hline
%			$\mathcal{B}$ & billiards layout\\
%            \hline
%            $sim(\cdot)$ &similarity measure for billiards layouts \\
%            \hline
%            $Net(\cdot)$ &shared network in BL2Vec model\\
%            \hline
%            $\mathcal{T}$ &token representation of $\mathcal{B}$\\
%            \hline
%            $x$ & $n \times K'$ embedded features\\
%            \hline
%            $v$  &  $K$-dimensional embedding vector of $\mathcal{B}$\\
%            \hline
%            $\mathcal{L}$  &  triplet loss\\
%            \hline
%	\end{tabular}
%\label{tab:notation}
%\vspace{-5mm}
%\end{table}
A billiards layout $\mathcal{B}$ as shown in Figure~\ref{fig:problem} corresponds to a rectangular pool table with six pockets and a set of balls $O$, where each ball $o \in O$ is associated with a spatial location $(x,y)$ on the table. 
% In a billiards game, there are one cue (white) ball and several object (colored) balls with the numbers.

Given two billiards layouts $\mathcal{B}_1$ and $\mathcal{B}_2$, we denote their similarity as $sim(\mathcal{B}_1, \mathcal{B}_2)$. Intuitively, the similarity function $sim(\cdot)$ should capture the locations of balls on the table. Figure \ref{fig:problem} illustrates an example of designing the similarity. $\mathcal{B}_q$ denotes a query layout, which contains a cue ball and three object balls 2,7,9. There are three different candidate layouts $\mathcal{B}_1$, $\mathcal{B}_2$ and $\mathcal{B}_3$. Among these candidate layouts, $\mathcal{B}_3$ is the most dissimilar to $\mathcal{B}_q$ since $\mathcal{B}_3$ contains totally different object balls (i.e., ball 3,4,6). Both $\mathcal{B}_1$ and $\mathcal{B}_2$ contain the same balls as $\mathcal{B}_q$; however, it is clear that the locations of the balls in $\mathcal{B}_1$ are more similar to those in $\mathcal{B}_q$ since these balls are located near to each other as they are in $\mathcal{B}_q$, while the balls in $\mathcal{B}_2$ are scattered. Therefore, while we do not know the exact values of these similarities, we tend to know a ranking of them (i.e., $sim(\mathcal{B}_q, \mathcal{B}_1) > sim(\mathcal{B}_q, \mathcal{B}_2) > sim(\mathcal{B}_q, \mathcal{B}_3)$). 

% In this paper, our goal is to design such $sim(\cdot)$ function for measuring the similarity among billiards layouts. We formulate the problem as follows.

% \subsection{Problem Statement} 
\smallskip\noindent\textbf{Problem Statement.}
Given a database of billiards layouts $\mathcal{D}$, we aim to map each billiards layout $\mathcal{B} \in \mathcal{D}$ to a low-dimensional space to capture similarities among billiards layouts. More specifically, for any two given billiards layouts $\mathcal{B}_1$ and $\mathcal{B}_2$, we map them to two $K$-dimensional vectors $v_1$ and $v_2$ via deep metric learning. The learned vectors should be similarity preserving, i.e., if two billiards layouts are similar, the Euclidean distance between their vectors would be small.

%Table~\ref{tab:notation} summarizes the notations that are frequently used in this paper.
}}


